Solving Rep-tile by Computers: Performance of Solvers and Analyses of Solutions

A rep-tile is a polygon that can be dissected into smaller copies (of the same size) of the original polygon. A polyomino is a polygon that is formed by joining one or more unit squares edge to edge. These two notions were first introduced and investigated by Solomon W. Golomb in the 1950s and popularized by Martin Gardner in the 1960s. Since then, dozens of studies have been made in communities of recreational mathematics and puzzles. In this study, we first focus on the specific rep-tiles that have been investigated in these communities. Since the notion of rep-tiles is so simple that can be formulated mathematically in a natural way, we can apply a representative puzzle solver, a MIP solver, and SAT-based solvers for solving the rep-tile problem in common. In comparing their performance, we can conclude that the puzzle solver is the weakest while the SAT-based solvers are the strongest in the context of simple puzzle solving. We then turn to analyses of the specific rep-tiles. Using some properties of the rep-tile patterns found by a solver, we can complete analyses of specific rep-tiles up to certain sizes. That is, up to certain sizes, we can determine the existence of solutions, clarify the number of the solutions, or we can enumerate all the solutions for each size. In the last case, we find new series of solutions for the rep-tiles which have never been found in the communities.

==> fig/revF-windmill-size15-jp-font-width.tex <==
┏━━━┳━━━┳┳━┳━━━┓　　　　　　　　　　　　　　┏━━━┳━━━┳━━━┳━┳┓　　　　　　　　　　　　　　　\\[-1pt]
┃┏┓┏╋┓┏┓┃┗┓┃┏┓┏┫　　　　　　　　　　　　　　┃┏┓┏┫┏┓┏┫┏┓┏┫┏┛┃　　　　　　　　　　　　　　　\\[-1pt]
┣┛┗┛┃┗┛┗┫┏┛┣┛┗┛┃　　　　　　　　　　　　　　┣┛┗┛┣┛┗┛┣┛┗┛┃┗┓┃　　　　　　　　　　　　　　　\\[-1pt]
┣━━━╋━━━┫┗┓┣┳━┳┫　　　　　　　　　　　　　　┣━━━╋━━━╋━━━┫┏┛┃　　　　　　　　　　　　　　　\\[-1pt]
┃┏┓┏┫┏┓┏┻┳╋┛┃┏┛┃　　　　　　　　　　　　　　┃┏┓┏┫┏┓┏╋┓┏┓┣┻┳┫　　　　　　　　　　　　　　　\\[-1pt]
┣┛┗┛┣┛┣┻┓┃┗┓┃┗┓┃　　　　　　　　　　　　　　┣┛┗┛┣┛┗┛┃┗┛┗┫┏┛┃　　　　　　　　　　　　　　　\\[-1pt]
┣━┳┳┻┓┃┏┛┃┏┛┃┏┛┃　　　　　　　　　　　　　　┣━┳┳╋━━━╋━━━┫┗┓┃　　　　　　　　　　　　　　　\\[-1pt]
┃┏┛┃┏┛┃┗┓┃┗┳┻┻━┫　　　　　　　　　　　　　　┃┏┛┃┗┓┏┓┃┏┓┏┫┏┛┃　　　　　　　　　　　　　　　\\[-1pt]
┃┗┓┃┗┳┫┏╋╋━╋┓┏┓┃　　　　　　　　　　　　　　┃┗┓┃┏┻┫┗╋┛┗┛┣┻┳┫　　　　　　　　　　　　　　　\\[-1pt]
┃┏┛┃┏┛┗┛┃┗┓┃┗┛┗┫　　　　　　　　　　　　　　┃┏┛┃┗┓┃┏┻┳┳━┫┏┛┃　　　　　　　　　　　　　　　\\[-1pt]
┣┻━┻╋━━━┫┏┛┣━━━┫　　　　　　　　　　　　　　┣╋━╋┳┛┃┗┓┃┗┓┃┗┓┃　　　　　　　　　　　　　　　\\[-1pt]
┣┓┏┓┃┏┓┏┫┗┓┃┏┓┏┫　　　　　　　　　　　　　　┃┗┓┃┗┓┣┳┛┃┏┛┃┏┛┃　　　　　　　　　　　　　　　\\[-1pt]
┃┗┛┗╋┛┗┛┣━╋╋┛┗┛┃　　　　　　　　　　　　　　┃┏┛┃┏┻┫┗┓┃┗┓┣╋━┫　　　　　　　　　　　　　　　\\[-1pt]
┣━━━╋━━━┫┏┛┣━━━┫　　　　　　　　　　　　　　┃┗┓┃┗┓┃┏┻╋┳┻┫┗┓┃　　　　　　　　　　　　　　　\\[-1pt]
┃┏┓┏╋┓┏┓┃┗┓┣┓┏┓┃　　　　　　　　　　　　　　┣━┻┻┳┛┃┗┓┃┗┓┃┏┛┃　　　　　　　　　　　　　　　\\[-1pt]
┣┛┗┛┃┗┛┗┫┏┛┃┗┛┗╋━┳━┳━━━┳━━━┳━━┻┓┏┓┣┓┣┳┛┃┏┛┃┗┓┣━━━┳━━━┳━━━┳━┳┓\\[-1pt]
┣━━━╋━━━╋┻━┻┳━━┻┓┃┏┻┓┏┓┣┓┏┓┣┓┏┓┣┫┗┛┗┫┗┓┃┗┓┣┳┻┫┏┓┏┫┏┓┏┫┏┓┏┫┏┛┃\\[-1pt]
┃┏┓┏┫┏┓┏┫┏┓┏┫┏┓┏┛┃┗┓┣┛┗┛┣┛┗┛┣┛┗┛┣━━━┫┏┻╋━╋┫┗┓┣┛┗┛┣┛┗┛┣┛┗┛┃┗┓┃\\[-1pt]
┣┛┗┛┣┛┣┛┗┛┣┛┗┛┣┻┓┃┏┛┣━━━╋━━━╋━━━┫┏┓┏┫┗┓┃┏┛┃┏┛┣━━━╋━━━╋━━━┫┏┛┃\\[-1pt]
┣━┳┳┻┓┣━━━╋━━━┫　┗┻┻┓┣┓┏┓┣┓┏┓┣┓┏┓┣┫┗┛┗┳┛┃┗┓┃┗┓┃┏┓┏╋┓┏┓┣┓┏┓┣┻┳┫\\[-1pt]
┃┏┛┃┏┛┣┓┏┓┣┓┏┓┃　　　　┣┛┣┛┗┛┣┛┗┛┣┛┗┛┣━━━╋┓┃┏┛┣━╋╋┛┗┛┃┗┛┗┫┗┛┗┫┏┛┃\\[-1pt]
┃┗┓┃┗┳┛┗┛┣┛┗┛┣┛　　　┏┻┓┣━━━╋━━━╋━━━┫┏┓┏┛┣┻┻━┫┏┛┣━━━╋━━━╋━━━┫┗┓┃\\[-1pt]
┃┏┛┃┏┻┳━┳╋━┳┳┫　　　　┃┏┛┣┓┏┓┣┓┏┓┣┓┏┓┣┛┣┻┓┣┓┏┓┃┗┓┃┏┓┏╋┓┏┓┃┏┓┏┫┏┛┃\\[-1pt]
┣╋━╋┻┓┃┏┛┃┏┛┃┗┳┳┓　┃┗┳┛┗┛┣┛┗┛┣┛┗┛┣┻┓┃┏┛┃┗┛┗┫┏┛┣┛┗┛┃┗┛┗╋┛┗┛┣┻┳┫\\[-1pt]
┃┗┓┃┏┛┃┗┓┃┗┓┃┏┛┃┗┳┫┏╋━━━╋━━━╋━━━┫┏┛┃┗┳┻━━┳┻┻━╋━━━╋━━━╋━━━┫┏┛┃\\[-1pt]
┃┏┛┃┗┓┃┏┛┃┏┛┃┗┓┃┏┛┗┛┃┏┓┏╋┓┏┓┣┓┏┓┃┗┳┫┏╋┓┏┓┃┏┓┏╋┓┏┓┃┏┓┏╋┓┏┓┃┗┓┃\\[-1pt]
┃┗┓┃┏╋┻╋┳┻╋━╋┳┛┃┗┳┳━╋┛┗┛┃┗┛┗┫┗┛┗┫┏┛┗┛┃┗┛┗╋┛┗┛┃┗┛┗╋┛┗┛┃┗┛┗┫┏┛┃\\[-1pt]
┣━┻┻┫┗┓┃┗┓┃┏┛┣━┻━┫┗┓┣━━━╋━━━╋━━━╋┻━━┳┻━━┳┻━━┳┻━━┳┻━━┳┻━━┳┻┻━┫\\[-1pt]
┃┏┓┏┫┏┛┃┏┛┃┗┓┣┓┏┓┃┏┛┣┓┏┓┃┏┓┏╋┓┏┓┃┏┓┏┫┏┓┏┫┏┓┏┫┏┓┏╋┓┏┓┃┏┓┏┫┏┓┏┫\\[-1pt]
┣┛┗┛┃┗┓┃┗┓┃┏┛┃┗┛┗┫┗┓┃┗┛┗╋┛┗┛┃┗┛┗╋┛┗┛┣┛┗┛┣┛┗┛┣┛┗┛┃┗┛┗╋┛┗┛┣┛┗┛┃\\[-1pt]
┗━━━┻━┻┻━┻┻┻━┻━━━┻━┻┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┛\\[-1pt]


==> fig/revF-windmill-size16-jp-font-width.tex <==
┏━━━┳┳━┳━┳┳━┳┳┳━┓　　　　　　　　　　　　　　　┏━━━┳━━━┳━━━┳━━━┓　　　　　　　　　　　　　　　　\\[-1pt]
┃┏┓┏┫┗┓┃┏┛┃┏┛┃┗┓┃　　　　　　　　　　　　　　　┃┏┓┏╋┓┏┓┃┏┓┏╋┓┏┓┃　　　　　　　　　　　　　　　　\\[-1pt]
┣┛┗┛┃┏┛┃┗┓┃┗┓┃┏┛┃　　　　　　　　　　　　　　　┣┛┗┛┃┗┛┗╋┛┗┛┃┗┛┗┫　　　　　　　　　　　　　　　　\\[-1pt]
┣┳━┳┫┗┓┃┏┛┃┏┛┃┗┓┃　　　　　　　　　　　　　　　┣━┳┳╋━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　\\[-1pt]
┃┗┓┃┗┳╋╋┻┳┻┻━╋┳┻┫　　　　　　　　　　　　　　　┃┏┛┃┗┓┏┓┃┏┓┏╋┓┏┓┃　　　　　　　　　　　　　　　　\\[-1pt]
┃┏┛┃┏┛┃┗┓┃┏┓┏┫┗┓┃　　　　　　　　　　　　　　　┃┗┓┃┏┻┫┗╋┛┗┛┃┗┛┗┫　　　　　　　　　　　　　　　　\\[-1pt]
┃┗┓┃┗┓┃┏┛┣┛┗┛┃┏┛┃　　　　　　　　　　　　　　　┃┏┛┃┗┓┃┏┻┳━━┻┳┳━┫　　　　　　　　　　　　　　　　\\[-1pt]
┣━┻┻┳┛┃┗┓┣━━━┫┗┓┃　　　　　　　　　　　　　　　┣┻━┻┳┛┃┗┓┃┏┓┏┫┗┓┃　　　　　　　　　　　　　　　　\\[-1pt]
┃┏┓┏╋┳┻┳┻╋┓┏┓┣┳┻┫　　　　　　　　　　　　　　　┣┓┏┓┣┓┣┳┛┣┛┗┛┃┏┛┃　　　　　　　　　　　　　　　　\\[-1pt]
┣┛┗┛┃┗┓┃┏┛┗┛┣┫┗┓┃　　　　　　　　　　　　　　　┃┗┛┗┫┗┛┗┓┣┳━┳┫┗┓┃　　　　　　　　　　　　　　　　\\[-1pt]
┣━━━┫┏┛┃┗┳┳┳┛┃┏┛┃　　　　　　　　　　　　　　　┣┳━┳┻━━┳╋┛┃┏┛┣┳┻┫　　　　　　　　　　　　　　　　\\[-1pt]
┣┓┏┓┃┗┓┃┏┛┃┗┓┃┗┓┃　　　　　　　　　　　　　　　┃┗┓┃┏┓┏┫┗┓┃┗┓┃┗┓┃　　　　　　　　　　　　　　　　\\[-1pt]
┃┗┛┗╋━╋╋┻┓┃┏┛┣┳┻┫　　　　　　　　　　　　　　　┃┏┛┣┛┗┛┃┏┛┃┏┛┃┏┛┃　　　　　　　　　　　　　　　　\\[-1pt]
┣━━━┫┏┛┃┏┛┃┗┳┫┗┓┃　　　　　　　　　　　　　　　┃┗┓┣━━━┫┗┳┻┻━┫┗┓┃　　　　　　　　　　　　　　　　\\[-1pt]
┃┏┓┏┫┗┓┃┗┳╋┳┛┃┏┛┃　　　　　　　　　　　　　　　┣━┻┻┓┏┓┣┳┫┏┓┏┻━┻┫　　　　　　　　　　　　　　　　\\[-1pt]
┣┛┗┛┃┏┛┃┏┛┃┗┓┃┗┓┃　　　　　　　　　　　　　　　┃┏┓┏╋┛┗┛┃┗┛┗┫┏┓┏┫　　　　　　　　　　　　　　　　\\[-1pt]
┣┳━┳┻┻━╋┻┓┃┏┛┣━┻┻┳━━━┳━━━┳━━━┳━━┻┫┗┛┗┳━━┻┳━━┻┫┗┛┗┳━━━┳━━━┳┳━┳━━━┓\\[-1pt]
┃┗┓┃┏┓┏┫┏┛┃┗┳┫┏┓┏┫┏┓┏┻┓┏┓┣┓┏┓┣┓┏┓┣┳┳━╋┓┏┓┣┓┏┓┣━━━┫┏┓┏┫┏┓┏┫┗┓┃┏┓┏┫\\[-1pt]
┃┏┛┣┛┗┛┃┗┳┻┳┛┗┛┣┛┗┛┣┻┓┣┛┗┛┣┛┗┛┣┛┗┛┃┗┓┃┗┛┗┫┗┛┗┫┏┓┏╋┛┗┛┣┛┗┛┃┏┛┣┛┗┛┃\\[-1pt]
┃┗┓┣━━━┫┏┻┓┣━━━╋━━━┫┏┛┣┳━┳┻┳┳┳┻┳━┳┫┏┛┣┳━┳╋━┳━╋┫┗┛┗┳━━┻┳━┳┫┗┓┣━━━┫\\[-1pt]
┣━┻┻┓┏┓┣┫┏┛┣┓┏┓┃┏┓┏┫┗┓┃┗┓┃┏┛┃┗┓┃┏┛┃┗┓┃┗┓┃┗┓┃┏┛┣━━━╋┓┏┓┃┏┛┣━╋┫┏┓┏┫\\[-1pt]
┣┓┏┓┣┛┗┛┃┗┓┃┗┛┗╋┛┗┛┃┏┻┫┏┛┃┗┓┃┏┛┃┗┓┣┳┻┫┏┛┃┏┛┃┗┓┃┏┓┏┫┗┛┗┫┗┓┃┏┛┣┛┗┛┃\\[-1pt]
┃┗┛┗╋┳━┳┫┏┻┻━┳━┻━┳━┻┛　┃┗┓┃┏┛┃┗┓┃┏┛┃┗┓┃┗┓┃┗┓┃┏┛┣┛┗┛┣━━━┫┏┛┃┗┓┣━━━┫\\[-1pt]
┣━━━┫┗┓┃┗┫┏┓┏┫┏┓┏┫　　　　┣━┻┻╋━┻━╋┻┻━┫┏┛┣━┻┻┳┻┻┻┳┻━━┳┫┏┓┏┻┻━┫┏┛┣┓┏┓┃\\[-1pt]
┃┏┓┏┫┏┛┃┏┻┫┗┛┗┫┗┛┗┓　　　┗┓┏┓┣┓┏┓┣┓┏┓┃┗┓┣┓┏┓┣┓┏┓┣┓┏┓┃┗┛┗┫┏┓┏╋╋━┫┗┛┗┫\\[-1pt]
┣┛┗┛┃┗┓┃┗┓┣━━━╋━━━┫　　　　┣┛┗┛┣┛┗┛┣┛┣╋━╋┫┗┛┗┫┗┛┗┫┗┛┗╋━━━╋┛┗┛┃┗┓┣━━━┫\\[-1pt]
┣━━━╋━┻┻┳┛┃┏┓┏┫┏┓┏┫　┏━━┻┳━━┻┳━━┻┓┃┗┓┃┗┳━━┻┳━━┻┳━━┻┓┏┓┣━━━┫┏┛┃┏┓┏┫\\[-1pt]
┣┓┏┓┣┓┏┓┣┓┣┫┗┛┗┫┗┛┗┳┫┏┓┏┫┏┓┏┫┏┓┏┛┃┏┛┃┏┻┓┏┓┣┓┏┓┣┓┏┓┣┫┗┫┏┓┏┫┗┓┣┛┗┛┃\\[-1pt]
┃┗┛┗┫┗┛┗┫┗┛┗┳┳━╋━┳┳┛┗┛┣┛┗┛┣┛┗┛┣╋━┫┗┓┃┗┓┣┛┗┛┣┛┗┛┣┛┗┛┃┏┻┫┗┛┗┳╋┻┳━┳┫\\[-1pt]
┣━━━╋━━━╋━━━┫┗┓┃┏┛┣━━━╋━━━╋━━━┫┗┓┣━┻┻┳┛┣━━━╋━━━╋━━━┫┗┓┣━━━┫┗┓┃┏┛┃\\[-1pt]
┃┏┓┏╋┓┏┓┣┓┏┓┃┏┛┃┗┓┣┓┏┓┣┓┏┓┣┓┏┓┃┏┛┃┏┓┏╋┓┣┓┏┓┣┓┏┓┣┓┏┓┣┳┛┃┏┓┏┫┏┛┃┗┓┃\\[-1pt]
┣┛┗┛┃┗┛┗┫┗┛┗┫┗┓┃┏┛┃┗┛┗┫┗┛┗┫┗┛┗┫┗┓┣┛┗┛┃┗┛┗┫┗┛┗┫┗┛┗┫┗┛┗┓┣┛┗┛┃┗┓┃┏┛┃\\[-1pt]
┗━━━┻━━━┻━━━┻━┻┻┻━┻━━━┻━━━┻━━━┻━┻┻━━━┻━━━┻━━━┻━━━┻━━━┻┻━━━┻━┻┻┻━┛\\[-1pt]


==> fig/revF-windmill-size17-jp-font-width.tex <==
┏┳━┳━┳┳━━━┳━┳┳━━━┓　　　　　　　　　　　　　　　　┏━━━┳━┳┳┳━┳━━━┳┳━┓　　　　　　　　　　　　　　　　　\\[-1pt]
┃┗┓┃┏┛┃┏┓┏┫┏┛┃┏┓┏┫　　　　　　　　　　　　　　　　┣┓┏┓┃┏┛┃┗┓┃┏┓┏┫┗┓┃　　　　　　　　　　　　　　　　　\\[-1pt]
┃┏┛┃┗┓┣┛┗┛┃┗┓┣┛┗┛┃　　　　　　　　　　　　　　　　┃┗┛┗┫┗┓┃┏┛┣┛┗┛┃┏┛┃　　　　　　　　　　　　　　　　　\\[-1pt]
┃┗┓┃┏┛┣━━━┫┏┛┣━━━┫　　　　　　　　　　　　　　　　┣━━━┫┏┛┃┗┓┣━━━┫┗┓┃　　　　　　　　　　　　　　　　　\\[-1pt]
┣━╋╋╋━┫┏┓┏╋╋━┫┏┓┏┫　　　　　　　　　　　　　　　　┣┓┏┓┣┻┳╋┳┻╋┓┏┓┣┳┻┫　　　　　　　　　　　　　　　　　\\[-1pt]
┃┏┛┃┗┓┣┛┗┛┃┗┓┣┛┗┛┃　　　　　　　　　　　　　　　　┃┗┛┗┫┏┛┃┗┓┃┗┫┗┛┗┓┃　　　　　　　　　　　　　　　　　\\[-1pt]
┃┗┓┃┏┛┣━━━┫┏┛┣━━━┫　　　　　　　　　　　　　　　　┣━━━┫┗┓┃┏┛┃┏┻━━┳┛┃　　　　　　　　　　　　　　　　　\\[-1pt]
┃┏┛┃┗┓┃┏┓┏┫┗┓┣┓┏┓┃　　　　　　　　　　　　　　　　┣┓┏┓┃┏┛┃┗┓┃┗┓┏┓┣┓┃　　　　　　　　　　　　　　　　　\\[-1pt]
┣╋━╋━┻┻┫┗┛┗┳┻┫┗┛┗┫　　　　　　　　　　　　　　　　┃┗┛┗╋┻━┻┳┻╋┳┻┫┗┛┗┫　　　　　　　　　　　　　　　　　\\[-1pt]
┃┗┓┣┓┏┓┣┳━┳┻┓┣━━━┫　　　　　　　　　　　　　　　　┣┳━┳┫┏┓┏┻┓┃┗┓┣━━━┫　　　　　　　　　　　　　　　　　\\[-1pt]
┃┏┛┃┗┫┗┛┗┓┃┏┛┃┏┓┏┫　　　　　　　　　　　　　　　　┃┗┓┃┗┛┗┫┏┛┃┏┛┃┏┓┏┫　　　　　　　　　　　　　　　　　\\[-1pt]
┃┗┓┃┏┻━━┳┛┃┗┓┣┛┗┛┃　　　　　　　　　　　　　　　　┃┏┛┣━━━┫┗┓┃┗┓┣┛┗┛┃　　　　　　　　　　　　　　　　　\\[-1pt]
┣━╋┫┗┓┏┓┣┓┃┏┻┻━┳━┫　　　　　　　　　　　　　　　　┃┗┓┣┓┏┓┃┏╋┻━┻╋━━━┫　　　　　　　　　　　　　　　　　\\[-1pt]
┃┏┛┣┳┻┫┗┛┗╋┫┏┓┏┻┓┃　　　　　　　　　　　　　　　　┣━╋┛┗┛┣╋┛┣┓┏┓┃┏┓┏┫　　　　　　　　　　　　　　　　　\\[-1pt]
┃┗┓┃┗┓┣━━━┫┗┛┗┫┏┛┃　　　　　　　　　　　　　　　　┃┏┻┳━┳┫┗┓┃┗┛┗╋┛┗┛┃　　　　　　　　　　　　　　　　　\\[-1pt]
┃┏┛┃┏┛┣┓┏┓┣━━━┫┗┓┃　　　　　　　　　　　　　　　　┃┗┓┃┏┛┃┏┛┣┳━━┻┳┳━┫　　　　　　　　　　　　　　　　　\\[-1pt]
┣╋━┫┗┓┃┗┛┗┫┏┓┏┫┏┻┫　　　　　　　　　　　　　　　　┃┏┛┃┗┓┃┗┳┛┃┏┓┏┫┗┓┃　　　　　　　　　　　　　　　　　\\[-1pt]
┃┗┓┣┳┻╋┳━━┻┫┗┛┗┫　┗━━┳━━━┳━━━┳━━━┳━┻┻┓┃┏┛┣┳┻┓┣┛┗┛┃┏┛┣━━━┳━━━┳━┳┳┳━┳━┳┓\\[-1pt]
┃┏┛┃┗┓┃┗┓┏┓┣━━━┫　　　　┣┓┏┓┣┓┏┓┣┓┏┓┃┏┓┏╋┻╋┳┛┃┏┛┣┳┳━┫┗┓┃┏┓┏╋┓┏┓┃┏┛┃┗┓┃┏┛┃\\[-1pt]
┃┗┓┃┏┛┃┏┻┫┗┫┏┓┏┛　　　┏┛┗┛┣┛┗┛┣┛┗┛┣┻┫┗┛┗┓┃┗┓┃┗┳┛┃┗┓┣┳┻╋┛┗┛┃┗┛┗┫┗┓┃┏┛┃┗┓┃\\[-1pt]
┣┳┻┫┗┓┃┗┓┃┏┻┫┗┫　　　　┣━━━╋━━━╋━━━┫┏┻━━┳┛┃┏┛┃┏┻┓┃┏┛┃┗┓┣━┳┳┻┳┳━┫┏┛┃┗┓┃┏┛┃\\[-1pt]
┃┗┓┣┳┻╋┳┛┃┗┓┃┏┻━━┓　┣┓┏┓┣┓┏┓┣┓┏┓┃┗┓┏┓┣┓┃┗┳┻┫┏┛┃┗┓┃┏┛┃┏┛┃┏┛┃┏┻╋━┻━╋┻┻━┫\\[-1pt]
┃┏┛┃┗┓┃┗┓┣┳┛┃┗┓┏┓┣┳┛┗┛┣┛┗┛┣┛┗┛┣┫┏╋┛┗┛┣┻━┻┓┃┗┳┻━┻┫┗┓┃┗┓┃┗┓┃┗┓┣┓┏┓┃┏┓┏┫\\[-1pt]
┃┗┓┃┏┛┃┏┻┫┗┓┣━╋┫┗┛┗┳━┳╋┳━┳┻┳┳━┫┗┛┗┳━┳┫┏┓┏┛┃┏┫┏┓┏╋┳┻┫┏┛┃┏┛┃┏┛┃┗┛┗╋┛┗┛┃\\[-1pt]
┣┳┻┫┗┓┃┗┓┃┏┻┫┏┛┣━━━┫┏┛┃┗┓┃┏┛┃┏┻┳┳━┫┏┛┗┛┣┻┓┣┛┗┛┣┛┃┗┓┣┻━┻╋━┻┻┓┣━━━╋━━━┫\\[-1pt]
┃┗┓┣━┻┻┳┛┃┗┓┃┗┓┣┓┏┓┃┗┓┃┏┛┃┗┓┃┗┓┃┗┓┃┗┳━━┻┓┣┻━━┳┻┓┃┏┛┃┏┓┏┫┏┓┏┻┫┏┓┏╋┓┏┓┃\\[-1pt]
┃┏┛┃┏┓┏╋┓┣┳┛┃┏┛┃┗┛┗┫┏┛┃┗┓┃┏┛┃┏┛┃┏┛┃┏┫┏┓┏┛┃┏┓┏┫┏┛┃┗┓┣┛┗┛┣┛┣┻┓┣┛┗┛┃┗┛┗┫\\[-1pt]
┃┗┓┣┛┗┛┃┗┛┗┓┣┻┳╋┳━┳╋┻┳┻┳╋┻╋┳┻╋┓┃┗┓┣┛┗┛┣┻┓┣┛┗┛┃┗┳╋┳┻╋━┳┳┻┓┃┏┛┣━━━╋━━━┫\\[-1pt]
┣━┻┻┳━━┻┳━━┻┫┏┛┃┗┓┃┗┓┃┏┛┃┏┛┃┏┛┣┻━┻╋━━━┫┏┻╋━━━┫┏┛┃┗┓┃┏┛┃┏┛┃┗┓┣┓┏┓┃┏┓┏┫\\[-1pt]
┣┓┏┓┃┏┓┏╋┓┏┓┃┗┓┃┏┛┃┏┛┃┗┓┃┗┓┃┗┓┣┓┏┓┣┓┏┓┃┗┓┣┓┏┓┣┻┓┃┏┛┃┗┓┃┗┳┫┏╋┫┗┛┗╋┛┗┛┃\\[-1pt]
┃┗┛┗╋┛┗┛┃┗┛┗┫┏┛┃┗┓┃┗┓┃┏┛┃┏┛┃┏┛┃┗┛┗┫┗┛┗┫┏┛┃┗┛┗┫┏┛┃┗┓┃┏┛┃┏┛┗┛┃┗┳┳━╋┳━┳┫\\[-1pt]
┣━━━╋━━━╋━━━╋┻━┻┳┻┻━╋┻┻━╋┻━┻╋━┻━┳━┻━┳━┻┻┓┣━━━┫┗┳┻━┻╋┻━┻╋━━━┫┏┛┃┏┛┃┏┛┃\\[-1pt]
┃┏┓┏╋┓┏┓┣┓┏┓┃┏┓┏┫┏┓┏┫┏┓┏┫┏┓┏╋┓┏┓┣┓┏┓┣┓┏┓┣┫┏┓┏┫┏┫┏┓┏┫┏┓┏┫┏┓┏┫┗┓┃┗┓┃┗┓┃\\[-1pt]
┣┛┗┛┃┗┛┗┫┗┛┗╋┛┗┛┣┛┗┛┣┛┗┛┣┛┗┛┃┗┛┗┫┗┛┗┫┗┛┗┫┗┛┗┫┗┛┗┫┗┛┗┫┗┛┗┫┗┛┗┳┛┃┏┛┃┏┛┃\\[-1pt]
┗━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━┻┻━┻┻━┛\\[-1pt]


==> fig/revF_8_00.tex <==
┏━━━┳━━━┓　　　　　　　┏━━━┳━━━┓　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┣━━━╋━━━┫　　　　　　　┣━━━╋━━━┫　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┣━━━╋━━━┫　　　　　　　┣━━━╋━━━┫　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　　┃　　　┣┳━━┳━━┳┛　　┏┛　　┏┻━┳━━┳━━┓\\[-1pt]
┣━━┳┻━┳━┛┃　　┃　　┣━━━╋━━━┫　　┃　　┃　　┃\\[-1pt]
┃　　┃　　┃　　┃　　┃　　┃　　　┃　　　┃　　┃　　┃　　┃\\[-1pt]
┃　　┃　　┃　　┃　　┃　　┃　　　┃　　　┃　　┃　　┃　　┃\\[-1pt]
┃　　┃　　┃　┏┻━┳┻━┳┻━┳━┻┳━━╋━━╋━━╋━━┫\\[-1pt]
┣━━┻┳━┻━┫　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃\\[-1pt]
┃　　　┃　　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃\\[-1pt]
┃　　　┃　　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃\\[-1pt]
┗━━━┻━━━┻━━┻━━┻━━┻━━┻━━┻━━┻━━┻━━┛\\[-1pt]


==> fig/revF_8_01.tex <==
┏━━━┳━━━┓　　　　　　　┏━━━┳━━━┓　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┣━━━╋━━━┫　　　　　　　┣━━━╋━━━┫　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┣━━━╋━━━┫　　　　　　　┣━━━╋━━━┫　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　　┃　　　┣━━┳━━┳┳┛　　┏┛　　┏┻━┳━━┳━━┓\\[-1pt]
┣━━┳╋━━━┫　　┃　　┃┗━┳━┻┳━━┫　　┃　　┃　　┃\\[-1pt]
┃　　┃┗┓　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃\\[-1pt]
┃　　┃　┗┓　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃\\[-1pt]
┃　　┃　　┃　┗┳━┻┳━┻┓　┃　　┃　　┣━━╋━━╋━━┫\\[-1pt]
┣━━┻┓　┃　　┃　　┃　　┣━┻━┳┻━━┫　　┃　　┃　　┃\\[-1pt]
┃　　　┃　┗┓　┃　　┃　　┃　　　┃　　　┃　　┃　　┃　　┃\\[-1pt]
┃　　　┃　　┗┓┃　　┃　　┃　　　┃　　　┃　　┃　　┃　　┃\\[-1pt]
┗━━━┻━━━┻┻━━┻━━┻━━━┻━━━┻━━┻━━┻━━┛\\[-1pt]


==> fig/revF_8_02.tex <==
┏━━━┳━━━┓　　　　　　　┏━━━┳━━━┓　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┣━━━╋━━━┫　　　　　　　┣━━━╋━━━┫　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┣━━━╋━━━┫　　　　　　　┣━━━╋━━━┫　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　　┃　　　┣━━┳━━┳┳┛　　┏┛　　┏┻━┳━━┳━━┓\\[-1pt]
┣━━━╋━━━┫　　┃　　┃┗━┳━┻┳━━┫　　┃　　┃　　┃\\[-1pt]
┃　　　┃　　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃\\[-1pt]
┃　　　┃　　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃\\[-1pt]
┣━━┳┻━┳━┻┳━┻┳━┻┓　┃　　┃　　┣━━╋━━╋━━┫\\[-1pt]
┃　　┃　　┃　　┃　　┃　　┣━┻━┳┻━━┫　　┃　　┃　　┃\\[-1pt]
┃　　┃　　┃　　┃　　┃　　┃　　　┃　　　┃　　┃　　┃　　┃\\[-1pt]
┃　　┃　　┃　　┃　　┃　　┃　　　┃　　　┃　　┃　　┃　　┃\\[-1pt]
┗━━┻━━┻━━┻━━┻━━┻━━━┻━━━┻━━┻━━┻━━┛\\[-1pt]


==> fig/revF_8_03.tex <==
┏━━━┳━━━┓　　　　　　　┏━━━┳━━━┓　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┣━━━╋━━━┫　　　　　　　┣━━━╋━━━┫　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┣━━━╋━━━┫　　　　　　　┣━━━╋━━━┫　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　　┃　　　┣┳━━┳━━┳┛　　┏┛　　┏┻━┳━━┳━━┓\\[-1pt]
┣━━┳┻━┳━┛┃　　┃　　┣━━━╋┳━━┫　　┃　　┃　　┃\\[-1pt]
┃　　┃　　┃　　┃　　┃　　┃　　┏┛┃　　┃　　┃　　┃　　┃\\[-1pt]
┃　　┃　　┃　　┃　　┃　　┃　┏┛　┃　　┃　　┃　　┃　　┃\\[-1pt]
┃　　┃　　┃　┏┻━┳┻━┳┛　┃　　┃　　┣━━╋━━╋━━┫\\[-1pt]
┣━━┻┳━┻━┫　　┃　　┃　　┃　┏┻━━┫　　┃　　┃　　┃\\[-1pt]
┃　　　┃　　　┃　　┃　　┃　┏┛　┃　　　┃　　┃　　┃　　┃\\[-1pt]
┃　　　┃　　　┃　　┃　　┃┏┛　　┃　　　┃　　┃　　┃　　┃\\[-1pt]
┗━━━┻━━━┻━━┻━━┻┻━━━┻━━━┻━━┻━━┻━━┛\\[-1pt]


==> fig/revF_8_04.tex <==
┏━━━┳━━━┓　　　　　　　┏━━━┳━━━┓　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┣━━━╋━━━┫　　　　　　　┣━━━╋━━━┫　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┣━━┳╋━━━┫　　　　　　　┣━━━╋━━━┫　　　　　　　　\\[-1pt]
┃　　┃┗┓　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　┃　┗┓　┗┳━━┳━━┳┛　　┏┛　　┏┻━┳━━┳━━┓\\[-1pt]
┃　　┃　　┃　　┃　　┃　　┣━━━╋━━━┫　　┃　　┃　　┃\\[-1pt]
┣━━┻┓　┃　　┃　　┃　　┃　　　┃　　　┃　　┃　　┃　　┃\\[-1pt]
┃　　　┃　┗┓　┃　　┃　　┃　　　┃　　　┃　　┃　　┃　　┃\\[-1pt]
┃　　　┃　　┗┳┻━┳┻━┳┻━┳━┻┳━━╋━━╋━━╋━━┫\\[-1pt]
┣━━━╋━━━┫　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃\\[-1pt]
┃　　　┃　　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃\\[-1pt]
┃　　　┃　　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃　　┃\\[-1pt]
┗━━━┻━━━┻━━┻━━┻━━┻━━┻━━┻━━┻━━┻━━┛\\[-1pt]


==> fig/revF_8_05.tex <==
┏━━━┳━━━┓　　　　　　　┏━━━┳━━━┓　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┣━━━╋━━━┫　　　　　　　┣━━━╋━━━┫　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┣━━┳╋━━━┫　　　　　　　┣━━━╋━━━┫　　　　　　　　\\[-1pt]
┃　　┃┗┓　　┃　　　　　　　┃　　　┃　　　┃　　　　　　　　\\[-1pt]
┃　　┃　┗┓　┗┳━━┳━━┳┛　　┏┛　　┏┻━┳━━┳━━┓\\[-1pt]
┃　　┃　　┃　　┃　　┃　　┣━━━╋┳━━┫　　┃　　┃　　┃\\[-1pt]
┣━━┻┓　┃　　┃　　┃　　┃　　┏┛┃　　┃　　┃　　┃　　┃\\[-1pt]
┃　　　┃　┗┓　┃　　┃　　┃　┏┛　┃　　┃　　┃　　┃　　┃\\[-1pt]
┃　　　┃　　┗┳┻━┳┻━┳┛　┃　　┃　　┣━━╋━━╋━━┫\\[-1pt]
┣━━━╋━━━┫　　┃　　┃　　┃　┏┻━━┫　　┃　　┃　　┃\\[-1pt]
┃　　　┃　　　┃　　┃　　┃　┏┛　┃　　　┃　　┃　　┃　　┃\\[-1pt]
┃　　　┃　　　┃　　┃　　┃┏┛　　┃　　　┃　　┃　　┃　　┃\\[-1pt]
┗━━━┻━━━┻━━┻━━┻┻━━━┻━━━┻━━┻━━┻━━┛\\[-1pt]


==> fig/revF_9_00.tex <==
┏━━┳━━┳━━┓　　　　　　　　┏━━┳━━┳━━┓　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━━╋━━┫　　　　　　　　┣━━╋━━╋━━┫　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━┻┳━┻┳━┫　　　　　　　　┣━━┻┳━┻┳━┫　　　　　　　　　\\[-1pt]
┃　　　┃　　┃　┗┳━━━┳━━━┫　　　┃　　┃　┗┳━━━┳━━━┓\\[-1pt]
┃　　　┃　　┃　　┃　　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃\\[-1pt]
┣━━┳┫　　┃　　┃　　　┃　　　┣━━━┫　　┃　　┃　　　┃　　　┃\\[-1pt]
┃　　┃┗┳━┻━┓┣━━━╋━━━╋┓　　┗┳━┻━┓┣━━━╋━━━┫\\[-1pt]
┃　　┃　┗┓　　┗┫　　　┃　　　┃┗┓　　┗┓　　┗┫　　　┃　　　┃\\[-1pt]
┃　　┃　　┃　　　┃　　　┃　　　┃　┗┳━━┫　　　┃　　　┃　　　┃\\[-1pt]
┣━━┻┓　┣━━━╋━━━╋━━━┫　　┃　　┣━━━╋━━━╋━━━┫\\[-1pt]
┃　　　┃　┗┓　　┗┓　　┗┓　　┗┓　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　┗┓　　┗┓　　┗┓　　┗┓┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┗━━━┻━━━┻━━━┻━━━┻━━━┻┻━━┻━━━┻━━━┻━━━┛\\[-1pt]


==> fig/revF_9_01.tex <==
┏━━┳━━┳━━┓　　　　　　　　┏━━┳━━┳━━┓　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━━╋━━┫　　　　　　　　┣━━╋━━╋━━┫　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━┻┳━┻┳━┫　　　　　　　　┣━━╋━┳┻━━┫　　　　　　　　　\\[-1pt]
┃　　　┃　　┃　┗┳━━━┳━━━┫　　┃　┗┓　　┗┳━━━┳━━━┓\\[-1pt]
┃　　　┃　　┃　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┣━━┳┫　　┃　　┃　　　┃　　　┃　　┃　　┣━━━┫　　　┃　　　┃\\[-1pt]
┃　　┃┗┳━┻━┓┣━━━╋━━━╋┳━┻━┓┃　　　┣━━━╋━━━┫\\[-1pt]
┃　　┃　┗┓　　┗┫　　　┃　　　┃┗┓　　┗┫　　　┃　　　┃　　　┃\\[-1pt]
┃　　┃　　┃　　　┃　　　┃　　　┃　┗┓　　┗┳━━┫　　　┃　　　┃\\[-1pt]
┣━━┻┓　┣━━━╋━━━╋━━━┫　　┣━━━┫　　┣━━━╋━━━┫\\[-1pt]
┃　　　┃　┗┓　　┗┓　　┗┓　　┗┓　┃　　　┃　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　┗┓　　┗┓　　┗┓　　┗┓┃　　　┃　　┃　　　┃　　　┃\\[-1pt]
┗━━━┻━━━┻━━━┻━━━┻━━━┻┻━━━┻━━┻━━━┻━━━┛\\[-1pt]


==> fig/revF_9_02.tex <==
┏━━┳━━┳━━┓　　　　　　　　┏━━┳━━┳━━┓　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━━╋━━┫　　　　　　　　┣━━╋━━╋━━┫　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━┻┳━┻┳━┫　　　　　　　　┣━━╋━┳┻━━┫　　　　　　　　　\\[-1pt]
┃　　　┃　　┃　┗┳━━━┳━━━┫　　┃　┗┓　　┗┳━━━┳━━━┓\\[-1pt]
┃　　　┃　　┃　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┣━━┳┫　　┃　　┃　　　┃　　　┃　　┃　　┣━━━┫　　　┃　　　┃\\[-1pt]
┃　　┃┗┳━┻━┓┣━━━╋━━━╋━━┻┳┓┃　　　┣━━━╋━━━┫\\[-1pt]
┃　　┃　┗┓　　┗┫　　　┃　　　┃　　　┃┗┫　　　┃　　　┃　　　┃\\[-1pt]
┃　　┃　　┃　　　┃　　　┃　　　┃　　　┃　┗┳━━┫　　　┃　　　┃\\[-1pt]
┣━━┻┓　┣━━━╋━━━╋━━━╋━━━┫　　┃　　┣━━━╋━━━┫\\[-1pt]
┃　　　┃　┗┓　　┗┓　　┗┓　　┗┓　　┗┓　┃　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　┗┓　　┗┓　　┗┓　　┗┓　　┗┓┃　　┃　　　┃　　　┃\\[-1pt]
┗━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻┻━━┻━━━┻━━━┛\\[-1pt]


==> fig/revF_9_03.tex <==
┏━━┳━━┳━━┓　　　　　　　　┏━━┳━━┳━━┓　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━━╋━━┫　　　　　　　　┣━━╋━━╋━━┫　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━┻┳━┻┳━┫　　　　　　　　┣━━┻┳━┻┳━┫　　　　　　　　　\\[-1pt]
┃　　　┃　　┃　┗┳━━━┳━━━┫　　　┃　　┃　┗┳━━━┳━━━┓\\[-1pt]
┃　　　┃　　┃　　┃　　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃\\[-1pt]
┣━━┳┫　　┃　　┃　　　┃　　　┣━━━┫　　┃　　┃　　　┃　　　┃\\[-1pt]
┃　　┃┗┳━┻━┓┣━━━╋┳━━┻┓　　┗┳━┻━┓┣━━━╋━━━┫\\[-1pt]
┃　　┃　┗┓　　┗┫　　　┃┗┓　　┗┓　　┗┓　　┗┫　　　┃　　　┃\\[-1pt]
┃　　┃　　┃　　　┃　　　┃　┗┓　　┗┳━━┫　　　┃　　　┃　　　┃\\[-1pt]
┣━━┻┓　┣━━━╋━━━┫　　┣━━━┫　　┣━━━╋━━━╋━━━┫\\[-1pt]
┃　　　┃　┗┓　　┗┓　　┗┓　┃　　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　┗┓　　┗┓　　┗┓┃　　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┗━━━┻━━━┻━━━┻━━━┻┻━━━┻━━┻━━━┻━━━┻━━━┛\\[-1pt]


==> fig/revF_9_04.tex <==
┏━━┳━━┳━━┓　　　　　　　　┏━━┳━━┳━━┓　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━━╋━━┫　　　　　　　　┣━━╋━━╋━━┫　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━┻┳━┻┳━┫　　　　　　　　┣━━┻┳━┻┳━┫　　　　　　　　　\\[-1pt]
┃　　　┃　　┃　┗┳━━━┳━━━┫　　　┃　　┃　┗┳━━━┳━━━┓\\[-1pt]
┃　　　┃　　┃　　┃　　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃\\[-1pt]
┣━━┳┫　　┃　　┃　　　┃　　　┣━━━┫　　┃　　┃　　　┃　　　┃\\[-1pt]
┃　　┃┗┳━┻━┓┣┳━━┻┳━━┻┓　　┗┳━┻━┓┣━━━╋━━━┫\\[-1pt]
┃　　┃　┗┓　　┗┫┗┓　　┗┓　　┗┓　　┗┓　　┗┫　　　┃　　　┃\\[-1pt]
┃　　┃　　┃　　　┃　┗┓　　┗┓　　┗┳━━┫　　　┃　　　┃　　　┃\\[-1pt]
┣━━┻┓　┣━━━┫　　┣━━━╋━━━┫　　┣━━━╋━━━╋━━━┫\\[-1pt]
┃　　　┃　┗┓　　┗┓　┃　　　┃　　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　┗┓　　┗┓┃　　　┃　　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┗━━━┻━━━┻━━━┻┻━━━┻━━━┻━━┻━━━┻━━━┻━━━┛\\[-1pt]


==> fig/revF_9_05.tex <==
┏━━┳━━┳━━┓　　　　　　　　┏━━┳━━┳━━┓　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━━╋━━┫　　　　　　　　┣━━╋━━╋━━┫　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━┳┻━━┫　　　　　　　　┣━━┻┳━┻┳━┫　　　　　　　　　\\[-1pt]
┃　　┃　┗┓　　┗┳━━━┳━━━┫　　　┃　　┃　┗┳━━━┳━━━┓\\[-1pt]
┃　　┃　　┃　　　┃　　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃\\[-1pt]
┃　　┃　　┣━━━┫　　　┃　　　┣━━━┫　　┃　　┃　　　┃　　　┃\\[-1pt]
┣━━┻┓　┗┓　　┗┳━━┻┳━━┻┓　　┗┳━┻━┓┣━━━╋━━━┫\\[-1pt]
┃　　　┃　　┗┓　　┗┓　　┗┓　　┗┓　　┗┓　　┗┫　　　┃　　　┃\\[-1pt]
┃　　　┣━━┳┻━┳━┻┓　　┗┓　　┗┳━━┫　　　┃　　　┃　　　┃\\[-1pt]
┣━━━┫　　┃　　┃　　┣━━━╋━━━┫　　┣━━━╋━━━╋━━━┫\\[-1pt]
┃　　　┃　　┃　　┃　　┃　　　┃　　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　┃　　┃　　┃　　　┃　　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┗━━━┻━━┻━━┻━━┻━━━┻━━━┻━━┻━━━┻━━━┻━━━┛\\[-1pt]


==> fig/revF_9_06.tex <==
┏━━┳━━┳━━┓　　　　　　　　┏━━┳━━┳━━┓　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━━╋━━┫　　　　　　　　┣━━╋━━╋━━┫　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━┻┳━┻┳━┫　　　　　　　　┣━━┻┳━┻┳━┫　　　　　　　　　\\[-1pt]
┃　　　┃　　┃　┗┳━━━┳━━━┫　　　┃　　┃　┗┳━━━┳━━━┓\\[-1pt]
┃　　　┃　　┃　　┃　　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃\\[-1pt]
┣━━━┫　　┃　　┃　　　┃　　　┣━━━┫　　┃　　┃　　　┃　　　┃\\[-1pt]
┃　　　┣━━┻┓　┗┳━━┻┳━━┻┓　　┗┳━┻━┓┣━━━╋━━━┫\\[-1pt]
┃　　　┃　　　┃　　┗┓　　┗┓　　┗┓　　┗┓　　┗┫　　　┃　　　┃\\[-1pt]
┣━━┳┛　　┏┻━┳━┻┓　　┗┓　　┗┳━━┫　　　┃　　　┃　　　┃\\[-1pt]
┃　　┣━━━┫　　┃　　┣━━━╋━━━┫　　┣━━━╋━━━╋━━━┫\\[-1pt]
┃　　┃　　　┃　　┃　　┃　　　┃　　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　┃　　　┃　　┃　　┃　　　┃　　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┗━━┻━━━┻━━┻━━┻━━━┻━━━┻━━┻━━━┻━━━┻━━━┛\\[-1pt]


==> fig/revF_9_07.tex <==
┏━━┳━━┳━━┓　　　　　　　　┏━━┳━━┳━━┓　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━━╋━━┫　　　　　　　　┣━━╋━━╋━━┫　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━┻┳━┻┳━┫　　　　　　　　┣━━┻┳━┻┳━┫　　　　　　　　　\\[-1pt]
┃　　　┃　　┃　┗┳━━━┳━━━┫　　　┃　　┃　┗┳━━━┳━━━┓\\[-1pt]
┃　　　┃　　┃　　┃　　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃\\[-1pt]
┣━━┳┫　　┃　　┃　　　┃　　　┣━━┳┫　　┃　　┃　　　┃　　　┃\\[-1pt]
┃　　┃┗┳━┻━┓┣━━━╋━━━┫　　┃┗┳━┻━┓┣━━━╋━━━┫\\[-1pt]
┃　　┃　┗┓　　┗┫　　　┃　　　┃　　┃　┗┓　　┗┫　　　┃　　　┃\\[-1pt]
┃　　┃　　┃　　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┣━━┻┓　┣━━━╋━━━╋━━━╋━━┻┓　┣━━━╋━━━╋━━━┫\\[-1pt]
┃　　　┃　┗┓　　┗┓　　┗┓　　┗┓　　┗┓┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　┗┓　　┗┓　　┗┓　　┗┓　　┗┫　　　┃　　　┃　　　┃\\[-1pt]
┗━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┛\\[-1pt]


==> fig/revF_9_08.tex <==
┏━━┳━━┳━━┓　　　　　　　　┏━━┳━━┳━━┓　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━━╋━━┫　　　　　　　　┣━━╋━━╋━━┫　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━┻┳━┻┳━┫　　　　　　　　┣━━╋━┳┻━━┫　　　　　　　　　\\[-1pt]
┃　　　┃　　┃　┗┳━━━┳━━━┫　　┃　┗┓　　┗┳━━━┳━━━┓\\[-1pt]
┃　　　┃　　┃　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┣━━┳┫　　┃　　┃　　　┃　　　┃　　┃　　┣━━━┫　　　┃　　　┃\\[-1pt]
┃　　┃┗┳━┻━┓┣━━━╋┳━━┻┳━┻━┓┃　　　┣━━━╋━━━┫\\[-1pt]
┃　　┃　┗┓　　┗┫　　　┃┗┓　　┗┓　　┗┫　　　┃　　　┃　　　┃\\[-1pt]
┃　　┃　　┃　　　┃　　　┃　┗┓　　┗┓　　┗┳━━┫　　　┃　　　┃\\[-1pt]
┣━━┻┓　┣━━━╋━━━┫　　┣━━━╋━━━┫　　┣━━━╋━━━┫\\[-1pt]
┃　　　┃　┗┓　　┗┓　　┗┓　┃　　　┃　　　┃　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　┗┓　　┗┓　　┗┓┃　　　┃　　　┃　　┃　　　┃　　　┃\\[-1pt]
┗━━━┻━━━┻━━━┻━━━┻┻━━━┻━━━┻━━┻━━━┻━━━┛\\[-1pt]


==> fig/revF_9_09.tex <==
┏━━┳━━┳━━┓　　　　　　　　┏━━┳━━┳━━┓　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━━╋━━┫　　　　　　　　┣━━╋━━╋━━┫　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━┻┳━┻┳━┫　　　　　　　　┣━━╋━┳┻━━┫　　　　　　　　　\\[-1pt]
┃　　　┃　　┃　┗┳━━━┳━━━┫　　┃　┗┓　　┗┳━━━┳━━━┓\\[-1pt]
┃　　　┃　　┃　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┣━━┳┫　　┃　　┃　　　┃　　　┃　　┃　　┣━━━┫　　　┃　　　┃\\[-1pt]
┃　　┃┗┳━┻━┓┣┳━━┻┳━━┻┳━┻━┓┃　　　┣━━━╋━━━┫\\[-1pt]
┃　　┃　┗┓　　┗┫┗┓　　┗┓　　┗┓　　┗┫　　　┃　　　┃　　　┃\\[-1pt]
┃　　┃　　┃　　　┃　┗┓　　┗┓　　┗┓　　┗┳━━┫　　　┃　　　┃\\[-1pt]
┣━━┻┓　┣━━━┫　　┣━━━╋━━━╋━━━┫　　┣━━━╋━━━┫\\[-1pt]
┃　　　┃　┗┓　　┗┓　┃　　　┃　　　┃　　　┃　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　┗┓　　┗┓┃　　　┃　　　┃　　　┃　　┃　　　┃　　　┃\\[-1pt]
┗━━━┻━━━┻━━━┻┻━━━┻━━━┻━━━┻━━┻━━━┻━━━┛\\[-1pt]


==> fig/revF_9_10.tex <==
┏━━┳━━┳━━┓　　　　　　　　┏━━┳━━┳━━┓　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━━╋━━┫　　　　　　　　┣━━╋━━╋━━┫　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━┳┻━━┫　　　　　　　　┣━━╋━┳┻━━┫　　　　　　　　　\\[-1pt]
┃　　┃　┗┓　　┗┳━━━┳━━━┫　　┃　┗┓　　┗┳━━━┳━━━┓\\[-1pt]
┃　　┃　　┃　　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　┃　　┣━━━┫　　　┃　　　┃　　┃　　┣━━━┫　　　┃　　　┃\\[-1pt]
┣━━┻┓　┗┓　　┗┳━━┻┳━━┻┳━┻━┓┃　　　┣━━━╋━━━┫\\[-1pt]
┃　　　┃　　┗┓　　┗┓　　┗┓　　┗┓　　┗┫　　　┃　　　┃　　　┃\\[-1pt]
┃　　　┣━━┳┻━┳━┻┓　　┗┓　　┗┓　　┗┳━━┫　　　┃　　　┃\\[-1pt]
┣━━━┫　　┃　　┃　　┣━━━╋━━━╋━━━┫　　┣━━━╋━━━┫\\[-1pt]
┃　　　┃　　┃　　┃　　┃　　　┃　　　┃　　　┃　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　┃　　┃　　┃　　　┃　　　┃　　　┃　　┃　　　┃　　　┃\\[-1pt]
┗━━━┻━━┻━━┻━━┻━━━┻━━━┻━━━┻━━┻━━━┻━━━┛\\[-1pt]


==> fig/revF_9_11.tex <==
┏━━┳━━┳━━┓　　　　　　　　┏━━┳━━┳━━┓　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━━╋━━┫　　　　　　　　┣━━╋━━╋━━┫　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━┻┳━┻┳━┫　　　　　　　　┣━━╋━┳┻━━┫　　　　　　　　　\\[-1pt]
┃　　　┃　　┃　┗┳━━━┳━━━┫　　┃　┗┓　　┗┳━━━┳━━━┓\\[-1pt]
┃　　　┃　　┃　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┣━━━┫　　┃　　┃　　　┃　　　┃　　┃　　┣━━━┫　　　┃　　　┃\\[-1pt]
┃　　　┣━━┻┓　┗┳━━┻┳━━┻┳━┻━┓┃　　　┣━━━╋━━━┫\\[-1pt]
┃　　　┃　　　┃　　┗┓　　┗┓　　┗┓　　┗┫　　　┃　　　┃　　　┃\\[-1pt]
┣━━┳┛　　┏┻━┳━┻┓　　┗┓　　┗┓　　┗┳━━┫　　　┃　　　┃\\[-1pt]
┃　　┣━━━┫　　┃　　┣━━━╋━━━╋━━━┫　　┣━━━╋━━━┫\\[-1pt]
┃　　┃　　　┃　　┃　　┃　　　┃　　　┃　　　┃　　┃　　　┃　　　┃\\[-1pt]
┃　　┃　　　┃　　┃　　┃　　　┃　　　┃　　　┃　　┃　　　┃　　　┃\\[-1pt]
┗━━┻━━━┻━━┻━━┻━━━┻━━━┻━━━┻━━┻━━━┻━━━┛\\[-1pt]


==> fig/revF_9_12.tex <==
┏━━┳━━┳━━┓　　　　　　　　┏━━┳━━┳━━┓　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━━╋━━┫　　　　　　　　┣━━╋━━╋━━┫　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━━┻┳━┫　　　　　　　　┣━━╋━┳┻━━┫　　　　　　　　　\\[-1pt]
┃　　┃　　　┃　┗┳━━━┳━━━┫　　┃　┗┓　　┗┳━━━┳━━━┓\\[-1pt]
┃　　┃　　　┃　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　┣━━━┫　　┃　　　┃　　　┃　　┃　　┣━━━┫　　　┃　　　┃\\[-1pt]
┣━━┻┓　　┗┓　┗┳━━┻┳━━┻┳━┻━┓┃　　　┣━━━╋━━━┫\\[-1pt]
┃　　　┃　　　┃　　┗┓　　┗┓　　┗┓　　┗┫　　　┃　　　┃　　　┃\\[-1pt]
┃　　　┣━━┳┻━┳━┻┓　　┗┓　　┗┓　　┗┳━━┫　　　┃　　　┃\\[-1pt]
┣━━━┫　　┃　　┃　　┣━━━╋━━━╋━━━┫　　┣━━━╋━━━┫\\[-1pt]
┃　　　┃　　┃　　┃　　┃　　　┃　　　┃　　　┃　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　┃　　┃　　┃　　　┃　　　┃　　　┃　　┃　　　┃　　　┃\\[-1pt]
┗━━━┻━━┻━━┻━━┻━━━┻━━━┻━━━┻━━┻━━━┻━━━┛\\[-1pt]


==> fig/revF_9_13.tex <==
┏━━┳━━┳━━┓　　　　　　　　┏━━┳━━┳━━┓　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━━╋━━┫　　　　　　　　┣━━╋━━╋━━┫　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　　　　　　　┃　　┃　　┃　　┃　　　　　　　　　\\[-1pt]
┣━━╋━━┻┳━┫　　　　　　　　┣━━┻┳━┻┳━┫　　　　　　　　　\\[-1pt]
┃　　┃　　　┃　┗┳━━━┳━━━┫　　　┃　　┃　┗┳━━━┳━━━┓\\[-1pt]
┃　　┃　　　┃　　┃　　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃\\[-1pt]
┃　　┣━━━┫　　┃　　　┃　　　┣━━━┫　　┃　　┃　　　┃　　　┃\\[-1pt]
┣━━┻┓　　┗┓　┗┳━━┻┳━━┻┓　　┗┳━┻━┓┣━━━╋━━━┫\\[-1pt]
┃　　　┃　　　┃　　┗┓　　┗┓　　┗┓　　┗┓　　┗┫　　　┃　　　┃\\[-1pt]
┃　　　┣━━┳┻━┳━┻┓　　┗┓　　┗┳━━┫　　　┃　　　┃　　　┃\\[-1pt]
┣━━━┫　　┃　　┃　　┣━━━╋━━━┫　　┣━━━╋━━━╋━━━┫\\[-1pt]
┃　　　┃　　┃　　┃　　┃　　　┃　　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　┃　　┃　　┃　　　┃　　　┃　　┃　　　┃　　　┃　　　┃\\[-1pt]
┗━━━┻━━┻━━┻━━┻━━━┻━━━┻━━┻━━━┻━━━┻━━━┛\\[-1pt]


==> fig/revJ-size18-2-rectocs.tex <==
┏━━┳━━┳━━┳━━┳━━┳━━┓　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　┃　　┃　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　┃　　┃　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　┃　　┃　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┣━━╋━━╋━━╋━━╋━━╋━━┫　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　┃　　┃　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　┃　　┃　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　┃　　┃　　┃　　┃　　┃　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┣━━┻┳━┻━┳┻━┳┻━━╋━━┫　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　┃　　　┃　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　┃　　　┃　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┣━━━╋━━━┫　　┣━━━┫　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┣━━┫　　　┣━━┫　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　┃　　　┃　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┣━━━╋━━━┫　　┣━━━┫　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　┃　　　┃　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┣━━┫　　　┣━━┫　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┣━━━╋━━━┫　　┣━━━┫　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　┃　　　┃　　┃　　　　　　　　　　　　　　　　　┏━━┳━━━┳━━━┳━━━┳━━┓\\[-1pt]
┃　　　┃　　　┃　　┃　　　┃　　┃　　　　　　　　　　　　　　　　　┃　　┃　　　┃　　　┃　　　┃　　┃\\[-1pt]
┣━━┳┻━┳━┻━┳┻━━┳┻━━┫　　　　　　　　　　　　　　　　　┃　　┃　　　┃　　　┃　　　┃　　┃\\[-1pt]
┃　　┃　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　┃　　┣━━━╋━━━╋━━━┫　　┃\\[-1pt]
┃　　┃　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　┣━━┫　　　┃　　　┃　　　┣━━┫\\[-1pt]
┃　　┃　　┣━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　　┃　　┃　　　┃　　　┃　　　┃　　┃\\[-1pt]
┣━━╋━━┫　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　┃　　┣━━┳┻━┳━┻┳━━┫　　┃\\[-1pt]
┃　　┃　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　┃　　┃　　┃　　┃　　┃　　┃　　┃\\[-1pt]
┃　　┃　　┣━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　　┣━━┫　　┃　　┃　　┃　　┣━━┫\\[-1pt]
┃　　┃　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　┃　　┃　　┃　　┃　　┃　　┃　　┃\\[-1pt]
┣━━╋━━┫　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　┃　　┣━━╋━━╋━━╋━━┫　　┃\\[-1pt]
┃　　┃　　┣━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　　┃　　┃　　┃　　┃　　┃　　┃　　┃\\[-1pt]
┃　　┃　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　┣━━┫　　┃　　┃　　┃　　┣━━┫\\[-1pt]
┃　　┃　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　┃　　┃　　┃　　┃　　┃　　┃　　┃\\[-1pt]
┣━━┻┳━┻━┳━┻━┳━┻┳━━┫　　　　　　　　　　　　　　　　　┃　　┣━━╋━━╋━━╋━━┫　　┃\\[-1pt]
┃　　　┃　　　┃　　　┃　　┃　　┃　　　　　　　　　　　　　　　　　┃　　┃　　┃　　┃　　┃　　┃　　┃\\[-1pt]
┃　　　┃　　　┃　　　┃　　┃　　┃　　　　　　　　　　　　　　　　　┣━━┫　　┃　　┃　　┃　　┣━━┫\\[-1pt]
┣━━━╋━━━╋━━━┫　　┃　　┃　　　　　　　　　　　　　　　　　┃　　┃　　┃　　┃　　┃　　┃　　┃\\[-1pt]
┃　　　┃　　　┃　　　┣━━┻┳━┻┳━━━┳━━┳━━━┳━━━┳━┻┓　┗┳━┻━┳┻━━╋━━┫　　┃\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　┃　　　┃　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃　　┃　　┃\\[-1pt]
┣━━┳┻━┳━┻┳━━┫　　　┃　　┃　　　┃　　┃　　　┃　　　┃　　┣━━┫　　　┃　　　┃　　┣━━┫\\[-1pt]
┃　　┃　　┃　　┃　　┣━━━┫　　┣━━━┫　　┣━━━╋━━━┫　　┃　　┣━━━╋━━━┫　　┃　　┃\\[-1pt]
┃　　┃　　┃　　┃　　┃　　　┣━━┫　　　┣━━┫　　　┃　　　┣━━┫　　┃　　　┃　　　┣━━┫　　┃\\[-1pt]
┃　　┃　　┃　　┃　　┃　　　┃　　┃　　　┃　　┃　　　┃　　　┃　　┃　　┃　　　┃　　　┃　　┃　　┃\\[-1pt]
┣━━╋━━╋━━╋━━┻┳━━┫　　┣━━━┫　　┣━━━╋━━━┫　　┣━━┻┳━━╋━━━┫　　┣━━┫\\[-1pt]
┃　　┃　　┃　　┃　　　┃　　┃　　┃　　　┃　　┃　　　┃　　　┃　　┃　　　┃　　┃　　　┃　　┃　　┃\\[-1pt]
┃　　┃　　┃　　┃　　　┃　　┣━━┫　　　┣━━┫　　　┃　　　┣━━┫　　　┃　　┃　　　┣━━┫　　┃\\[-1pt]
┃　　┃　　┃　　┣━━━┫　　┃　　┣━━━┫　　┣━━━╋━━━┫　　┣━━━┫　　┣━━━┫　　┃　　┃\\[-1pt]
┣━━╋━━╋━━┫　　　┣━━┫　　┃　　　┃　　┃　　　┃　　　┃　　┃　　　┣━━┫　　　┃　　┣━━┫\\[-1pt]
┃　　┃　　┃　　┃　　　┃　　┃　　┃　　　┃　　┃　　　┃　　　┃　　┃　　　┃　　┃　　　┃　　┃　　┃\\[-1pt]
┃　　┃　　┃　　┣━━━┫　　┣━━┻┳━━┻┳━┻━┳━┻━┳━┻━┳┻━━┳┛　┏┻━━┳┻━━┫　　┃\\[-1pt]
┃　　┃　　┃　　┃　　　┃　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　┃　　　┃　　　┃　　┃\\[-1pt]
┣━━╋━━╋━━┫　　　┣━━┫　　　┃　　　┃　　　┃　　　┃　　　┃　　　┣━━┫　　　┃　　　┣━━┫\\[-1pt]
┃　　┃　　┃　　┣━━━┫　　┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫　　┣━━━╋━━━┫　　┃\\[-1pt]
┃　　┃　　┃　　┃　　　┃　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　┃　　　┃　　　┃　　┃\\[-1pt]
┃　　┃　　┃　　┃　　　┃　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　┃　　　┃　　　┃　　┃\\[-1pt]
┗━━┻━━┻━━┻━━━┻━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━┻━━━┻━━━┻━━┛\\[-1pt]


==> fig/revJ-size24-rectocs.tex <==
┏━━━┳━━━┳━━━┳━━━┳━━━┳━━━┓　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　　\\[-1pt]
┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　　　　　　　　┏━━━┳━━━┳━━━┳━━━┳━━━┳━━━┓\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃\\[-1pt]
┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　　　　　　　　┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃\\[-1pt]
┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　　　　　　　　┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃\\[-1pt]
┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　　　　　　　　┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃\\[-1pt]
┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　　　　　　　　┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃\\[-1pt]
┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫　　　　　　　　　　　　　　　　　　　　　　　┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃\\[-1pt]
┣━━━╋━━┳┻━┳━┻┳━━┻┳━━╋━━━┫　　　　　　　　　　　　　　　　　　　　　　　┣━━┳┻━━┳┻━┳━┻┳━━┻┳━━╋━━━┫\\[-1pt]
┃　　　┃　　┃　　┃　　┃　　　┃　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　┃　　┃　　　┃　　┃　　┃　　　┃　　┃　　　┃\\[-1pt]
┃　　　┃　　┃　　┃　　┃　　　┃　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　┃　　┃　　　┃　　┃　　┃　　　┃　　┃　　　┃\\[-1pt]
┣━━━┫　　┃　　┃　　┣━━━┫　　┣━━━┫　　　　　　　　　　　　　　　　　　　　　　　┃　　┣━━━┫　　┃　　┣━━━┫　　┣━━━┫\\[-1pt]
┃　　　┣━━╋━━╋━━┫　　　┣━━┫　　　┃　　　　　　　　　　　　　　　　　　　　　　　┣━━┫　　　┣━━╋━━┫　　　┣━━┫　　　┃\\[-1pt]
┃　　　┃　　┃　　┃　　┃　　　┃　　┃　　　┃　　　　　　　　　　　　　　　　　　　　　　　┃　　┃　　　┃　　┃　　┃　　　┃　　┃　　　┃\\[-1pt]
┣━━━┫　　┃　　┃　　┣━━┳┛　┏┻━━┳┻━━┳━━━┳━━━┳━━━┳━━━┳━━━┳┛　┏┻━┳━┻┓　┗┓　┗┳━━┻┓　┗┳━━┫\\[-1pt]
┃　　　┃　　┃　　┃　　┃　　┃　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　┃　　┃　　┃　　┃　　┃　　　┃　　┃　　┃\\[-1pt]
┃　　　┣━━╋━━╋━━┫　　┣━━┫　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┣━━┫　　┃　　┣━━╋━━┫　　　┣━━┫　　┃\\[-1pt]
┣━━━┫　　┃　　┃　　┃　　┃　　┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫　　┃　　┃　　┃　　┃　　┣━━━┫　　┃　　┃\\[-1pt]
┃　　　┃　　┃　　┃　　┣━━┫　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　┣━━╋━━┫　　┃　　┃　　　┃　　┣━━┫\\[-1pt]
┃　　　┃　　┃　　┃　　┃　　┃　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　┃　　┃　　┃　　┃　　┃　　　┃　　┃　　┃\\[-1pt]
┣━━━╋━━╋━━┻┳━┻┓　┗┳━┻━┳━┻┳━━┻┳━━╋━━━╋━━┳┻━━┳┻━━┳┻━━┫　　┃　　┣━━╋━━╋━━┳┻━━┫　　┃\\[-1pt]
┃　　　┃　　┃　　　┃　　┃　　┃　　　┃　　┃　　　┃　　┃　　　┃　　┃　　　┃　　　┃　　　┃　　┃　　┃　　┃　　┃　　┃　　　┃　　┃\\[-1pt]
┃　　　┃　　┃　　　┃　　┣━━┫　　　┃　　┃　　　┃　　┃　　　┃　　┃　　　┃　　　┃　　　┣━━╋━━┫　　┃　　┃　　┃　　　┣━━┫\\[-1pt]
┣━━━┫　　┣━━━┫　　┃　　┣━━━┫　　┣━━━┫　　┣━━━┫　　┣━━━╋━━━╋━━━┫　　┃　　┃　　┃　　┃　　┣━━━┫　　┃\\[-1pt]
┃　　　┣━━┫　　　┣━━┫　　┃　　　┣━━┫　　　┣━━┫　　　┣━━┫　　　┃　　　┃　　　┃　　┃　　┣━━╋━━╋━━┫　　　┃　　┃\\[-1pt]
┃　　　┃　　┃　　　┃　　┃　　┃　　　┃　　┃　　　┃　　┃　　　┃　　┃　　　┃　　　┃　　　┃　　┃　　┃　　┃　　┃　　┃　　　┃　　┃\\[-1pt]
┣━━━┫　　┣━━━┫　　┣━━┻┳━━┻┓　┗┳━━┻┓　┗┳━━┻┓　┗┳━━┻┳━━┻┳━━┻┳━┻━┳┛　┏┛　┏┛　┏┻━━┳┻━━┫\\[-1pt]
┃　　　┃　　┃　　　┃　　┃　　　┃　　　┃　　┃　　　┃　　┃　　　┃　　┃　　　┃　　　┃　　　┃　　　┃　　┃　　┃　　┃　　　┃　　　┃\\[-1pt]
┃　　　┣━━┫　　　┣━━┫　　　┃　　　┣━━┫　　　┣━━┫　　　┣━━┫　　　┃　　　┃　　　┃　　　┣━━╋━━╋━━┫　　　┃　　　┃\\[-1pt]
┣━━━┫　　┣━━━┫　　┣━━━╋━━━┫　　┣━━━┫　　┣━━━┫　　┣━━━╋━━━╋━━━╋━━━┫　　┃　　┃　　┣━━━╋━━━┫\\[-1pt]
┃　　　┃　　┃　　　┃　　┃　　　┃　　　┃　　┃　　　┃　　┃　　　┃　　┃　　　┃　　　┃　　　┃　　　┃　　┃　　┃　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　┃　　　┃　　┃　　　┃　　　┃　　┃　　　┃　　┃　　　┃　　┃　　　┃　　　┃　　　┃　　　┃　　┃　　┃　　┃　　　┃　　　┃\\[-1pt]
┣━━━╋━━┻┳━━┻┳━┻━┳━┻━┳━┻━┳┻━━┳┻━━╋━━━╋━━┻┳━━┻┳━━┻┳━━┻┳━━┻┳━┻━┳┻━━╋━━━╋━━━┫\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃\\[-1pt]
┣━━━╋━━━╋━━━╋━━━╋━━━╋━━━╋━━━╋━━━╋━━━╋━━━╋━━━╋━━━╋━━━╋━━━╋━━━╋━━━╋━━━╋━━━┫\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃\\[-1pt]
┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃　　　┃\\[-1pt]
┗━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┻━━━┛\\[-1pt]


==> fig/revS-size11.tex <==
\begin{figure*}[htb]
\centering

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt07.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt08.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt09.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt12.tex}\end{tabular}}
}

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt13.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt14.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt15.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt16.tex}\end{tabular}}
}

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt17.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt18.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt19.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt22.tex}\end{tabular}}
}

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt23.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt24.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt25.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt26.tex}\end{tabular}}
}

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt27.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt28.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt29.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt30.tex}\end{tabular}}
}

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt46.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt47.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt48.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt55.tex}\end{tabular}}
}

\caption{階段型6-オミノ$k=11$のときの解の一覧(1/4)}
\label{fig:stair-i}
\end{figure*}

\begin{figure*}[htb]
\centering
\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt56.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt57.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt58.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt59.tex}\end{tabular}}
}

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt60.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt61.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt62.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt63.tex}\end{tabular}}
}

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt64.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt66.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt67.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt68.tex}\end{tabular}}
}

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt69.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt70.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt71.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt72.tex}\end{tabular}}
}

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt73.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-58-1-1-tex/revS-size11-all-list.txt74.tex}\end{tabular}}
}
\caption{階段型6-オミノ$k=11$のときの解の一覧(2/4)}
\label{fig:stair-ii}
\end{figure*}

\begin{figure*}[htb]
\centering
\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt01.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt02.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt03.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt04.tex}\end{tabular}}
}

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt05.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt06.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt10.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt11.tex}\end{tabular}}
}

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt20.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt21.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt31.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt32.tex}\end{tabular}}
}

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt33.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt34.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt35.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt36.tex}\end{tabular}}
}

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt37.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt38.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt39.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt40.tex}\end{tabular}}
}

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt41.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt42.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt43.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt44.tex}\end{tabular}}
}
\caption{階段型6-オミノ$k=11$のときの解の一覧(3/4)}
\label{fig:stair-iii}
\end{figure*}

\begin{figure*}[htb]
\centering
\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt45.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt49.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt50.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt51.tex}\end{tabular}}
}

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt52.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt53.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt54.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt65.tex}\end{tabular}}
}

\scalebox{0.7}{
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt75.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt76.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt77.tex}\end{tabular}}
{\tiny\begin{tabular}{l}\input{fig/sol-59-0-1-tex/revS-size11-all-list.txt78.tex}\end{tabular}}
}
\caption{階段型6-オミノ$k=11$のときの解の一覧(4/4)}
\label{fig:stair-iv}
\end{figure*}
